Exploring Feature Importance and Explainability Towards Enhanced ML-Based DoS Detection in AI Systems

Denial of Service (DoS) attacks pose a significant threat in the realm of AI systems security, causing substantial financial losses and downtime. However, AI systems' high computational demands, dynamic behavior, and data variability make monitoring and detecting DoS attacks challenging. Nowadays, statistical and machine learning (ML)-based DoS classification and detection approaches utilize a broad range of feature selection mechanisms to select a feature subset from networking traffic datasets. Feature selection is critical in enhancing the overall model performance and attack detection accuracy while reducing the training time. In this paper, we investigate the importance of feature selection in improving ML-based detection of DoS attacks. Specifically, we explore feature contribution to the overall components in DoS traffic datasets by utilizing statistical analysis and feature engineering approaches. Our experimental findings demonstrate the usefulness of the thorough statistical analysis of DoS traffic and feature engineering in understanding the behavior of the attack and identifying the best feature selection for ML-based DoS classification and detection.

==> refs.tex <==
@misc{DoS-harm,
  title = {How Much Will a \mbox{DDoS} Attack Cost Your Business?},
  howpublished = {\url{https://www.cloudbric.com/blog/2021/01/business-ddos-attacks-damages-and-cost/}},
  note = {Accessed: 2022-02-09}
}

@misc{lycos,
  title = {Intrusion Detection Evaluation Dataset (LYCOS-IDS2017)},
  url = {https://lycos-ids.univ-lemans.fr},
  note = {Accessed: April, 2023}
}

@article{jazi2017detecting,
  title={Detecting \mbox{HTTP}-based application layer \mbox{DoS} attacks on web servers in the presence of sampling},
  author={Jazi, Hossein Hadian and Gonzalez, Hugo and Stakhanova, Natalia and Ghorbani, Ali A.},
  journal={Computer Networks},
  volume={121},
  pages={25--36},
  year={2017},
  publisher={Elsevier}
}

@article{chin2018kernel,
  title={Kernel-Space Intrusion Detection Using Software-Defined Networking},
  author={Chin, Tommy and Xiong, Kaiqi and Rahouti, Mohamed},
  journal={EAI Endorsed Transactions on Security and Safety},
  volume={5},
  number={15},
  pages={e2},
  year={2018}
}

@article{rahouti2021synguard,
  title={\mbox{SYNGuard}: Dynamic threshold-based \mbox{SYN} flood attack detection and mitigation in software-defined networks},
  author={Rahouti, Mohamed and Xiong, Kaiqi and Ghani, Nasir and Shaikh, Farooq},
  journal={IET Networks},
  volume={10},
  number={2},
  pages={76--87},
  year={2021},
  publisher={Wiley Online Library}
}

@article{zheng2018realtime,
  title={Realtime \mbox{DDoS} defense using \mbox{COTS SDN} switches via adaptive correlation analysis},
  author={Zheng, Jing and Li, Qi and Gu, Guofei and Cao, Jiahao and Yau, \mbox{ David K.Y.} and Wu, Jianping},
  journal={TIFS},
  volume={13},
  number={7},
  pages={1838--1853},
  year={2018, IEEE},
  publisher={IEEE}
}

@article{david2021discriminating,
  title={Discriminating flash crowds from \mbox{DDoS} attacks using efficient thresholding algorithm},
  author={David, Jisa and Thomas, Ciza},
  journal={JPDC},
  volume={152},
  pages={79--87},
  year={2021, Elsevier}
}

@article{yu2011discriminating,
  title={Discriminating \mbox{DDoS} attacks from flash crowds using flow correlation coefficient},
  author={Yu, Shui and Zhou, Wanlei and Jia, Weijia and Guo, Song and Xiang, Yong and Tang, Feilong},
  journal={TPDS},
  volume={23},
  number={6},
  pages={1073--1080},
  year={2011, IEEE}
}

@inproceedings{rosay2022network,
  title={Network intrusion detection: A comprehensive analysis of CIC-IDS2017},
  author={Rosay, Arnaud and Cheval, Elo{\"\i}se and Carlier, Florent and Leroux, Pascal},
  booktitle={ICISSP},
  pages={25--36},
  year={2022},
  organization={SCITEPRESS-Science and Technology Publications}
}

@inproceedings{saha2022towards,
  title={Towards an Optimal Feature Selection Method for \mbox{AI}-Based \mbox{DDoS} Detection System},
  author={Saha, Sajal and Priyoti, Annita Tahsin and Sharma, Aakriti and Haque, Anwar},
  booktitle={CCNC},
  pages={425--428},
  year={2022},
  organization={IEEE}
}

@article{sarhan2022evaluating,
  title={Evaluating standard feature sets towards increased generalisability and explainability of  \mbox{ML}-based network intrusion detection},
  author={Sarhan, Mohanad and Layeghy, Siamak and Portmann, Marius},
  journal={Big Data Research},
  volume={30},
  pages={100359},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{sanchez2021feature,
  title={Feature selection evaluation towards a lightweight deep learning \mbox{DDoS} detector},
  author={Sanchez, Odnan Ref and Repetto, Matteo and Carrega, Alessandro and Bolla, Raffaele and Pajo, Jane Frances},
  booktitle={ICC},
  pages={1--6},
  year={2021},
  organization={IEEE}
}

@article{di2021supervised,
  title={Supervised feature selection techniques in network intrusion detection: A critical review},
  author={Di Mauro, Mario and Galatro, Giovanni and Fortino, Giancarlo and Liotta, Antonio},
  journal={Engineering Applications of Artificial Intelligence},
  volume={101},
  pages={104216},
  year={2021, Elsevier}
}

@inproceedings{setitra2022feature,
  title={Feature Modeling and Dimensionality Reduction to Improve \mbox{ML}-Based \mbox{DDoS} Detection Systems in SDN Environment},
  author={Setitra, Mohamed Ali and Benkhaddra, Ilyas and Bensalem, Zine El Abidine and Fan, Mingyu},
  booktitle={ICCWAMTIP},
  pages={1--7},
  year={2022},
  organization={IEEE}
}

@article{thakkar2021attack,
  title={Attack classification using feature selection techniques: a comparative study},
  author={Thakkar, Ankit and Lohiya, Ritika},
  journal={JAIHC},
  volume={12},
  pages={1249--1266},
  year={2021, Springer}
}

@inproceedings{liang2019empirical,
  title={An empirical study of intelligent approaches to \mbox{DDoS} detection in large scale networks},
  author={Liang, Xiaoyu and Znati, Taieb},
  booktitle={ICNC},
  pages={821--827},
  year={2019},
  organization={IEEE}
}

@inproceedings{rosay2021cic,
  author = {Rosay, Arnaud and Carlier, Florent and Cheval, Eloïse and Leroux, Pascal},
  title = {From {CIC-IDS2017} to {LYCOS-IDS2017}: A Corrected Dataset for Better Performance},
  booktitle = {IEEE/WIC/ACM WI-IAT},
  location = {Essendon, VIC, Australia},
  publisher = {ACM},
  year = {2021},
  isbn = {978-1-4503-8886-0},
  doi = {10.1145/3486622.3493973},
  pages = {6},
  numpages = {6},
  url = {https://doi.org/10.1145/3486622.3493973},
}

@inproceedings{sharafaldin2018toward,
  title={Toward Generating a New Intrusion Detection Dataset and Intrusion Traffic Characterization},
  author={Sharafaldin, Iman and Lashkari, Arash Habibi and Ghorbani, Ali A},
  booktitle={ICISSP},
  year={2018},
  month={January},
  address = {Portugal}
}

